Reliable Probability Intervals For Classification Using Inductive Venn Predictors Based on Distance Learning

Deep neural networks are frequently used by autonomous systems for their ability to learn complex, non-linear data patterns and make accurate predictions in dynamic environments. However, their use as black boxes introduces risks as the confidence in each prediction is unknown. Different frameworks have been proposed to compute accurate confidence measures along with the predictions but at the same time introduce a number of limitations like execution time overhead or inability to be used with high-dimensional data. In this paper, we use the Inductive Venn Predictors framework for computing probability intervals regarding the correctness of each prediction in real-time. We propose taxonomies based on distance metric learning to compute informative probability intervals in applications involving high-dimensional inputs. Empirical evaluation on image classification and botnet attacks detection in Internet-of-Things (IoT) applications demonstrates improved accuracy and calibration. The proposed method is computationally efficient, and therefore, can be used in real-time.

==> related_work.tex <==
\section{Related Work}
\label{sec:related_work}
% As modern LEC architectures get bigger in size to make predictions on data with increasingly levels of abstraction 
The estimation of reliable predictive uncertainty has become an important part of many modern machine learning components used in safety-critical applications. The first developments in computing uncertainty metrics happened in forecasting~\cite{ANewVectorPartitionoftheProbabilityScore,degroot1983comparison}. Since then different approaches have been proposed to make LEC predictions well-calibrated. Modern DNN architectures that use a softmax layer to produce a probability distribution over the output classes tend to be poorly calibrated and overconfident. Some of the approaches in producing well-calibrated models propose new training methods. In~\cite{pereyra2017regularizing}, the authors add a negative entropy term to the negative log-likelihood during training to penalize low-entropy output distributions. In~\cite{pmlr-v80-kumar18a}, calibration is achieved during the model training by minimizing the proposed Maximum Mean Calibration Error (MMCE). These methods require for a model to be trained with the calibration properties in mind and this may not be an option in pre-trained models. 

Another category of calibration methods proposes ways of post-processing the outputs of already trained models to produce calibrated confidence measures. The parametric methods assume that the  probabilities follow certain well-known  distributions whose parameters are to be estimated from the training data. The Platt's scaling method~\cite{Platt99probabilisticoutputs} is proposed for the calibration of Support Vector Machine (SVM) outputs. After the training of an SVM, the method computes the parameters of a sigmoid function to map the outputs into probabilities. Two extensions are the Piecewise Logistic Regression~\cite{zhang2004probabilistic} and the Temperature Scaling~\cite{Guo:2017:CMN:3305381.3305518}. The former assumes that the log-odds of calibrated probabilities follow a piecewise linear function and was proposed to be used with Naive Bayes, linear SVM and logistic regression classifiers. On the other hand, temperature scaling can be applied in DNNs with a softmax output layer. After the training of a DNN, a temperature scaling factor $T$ is computed on a validation set to scale the softmax outputs. However, in~\cite{kumar2019verified,ovadia2019can}, it is shown that Platt's scaling and temperature scaling are not as well calibrated as it is reported especially when the validation data are not independent and identically distributed (IID) and in the presence of distribution shifts. 

The Conformal Prediction (CP) framework is developed to compute prediction sets to satisfy a desired significance level~\cite{Vovk:2005:ALR:1062391,Shafer:2008:TCP:1390681.1390693,balasubramanian2014conformal}. Using CP together with methods that require long training times, such as DNNs, is computationally inefficient. In \cite{papadopoulos2007conformal} the authors suggest a modified version of the CP framework, they call Inductive Conformal Prediction (ICP), that has less computational overhead. The use of appropriate representations with ICP has been investigated in~\cite{papernot2018deep,boursinos2020assurance,boursinos2020trusted} where the results show better robustness, efficiency and real-time capabilities. However, the confidence assigned to each class is in the form of p-values which is less intuitive than probabilities.

% Confidence and uncertainty estimation in neural networks has received considerable attention especially in the context of classification tasks in computer vision~\cite{Guo:2017:CMN:3305381.3305518}. 

==> siamese.tex <==
\section{Siamese Network}
\label{sec:siamese}

\begin{figure}[ht]
\centering
\input{images/siamese.tikz}
\caption{Siamese network structure}
\label{fig:siamese_architecture}
\end{figure}

Central to the VP framework is the definition of the Venn taxonomy. This is a way of clustering of data points into a number of categories based on their similarity and is based on an underlying algorithm. For example a taxonomy can be defined to put in the same category examples that are classified in the same class by a DNN. The main idea of our approach is that the taxonomy can be defined efficiently by learning representations of the inputs for which the Euclidean distance is a suitable measure of similarity. The \textit{siamese network} is a DNN architecture that is trained to compute appropriate representations for distance metric learning~\cite{hadsell2006dimensionality,koch2015siamese}.

A siamese network is composed using two copies of the same neural network with shared parameters as shown in Fig.~\ref{fig:siamese_architecture}. Unlike training of classifiers where the label of each data point is a particular class, in distance metric learning pairs of data points are annotated either as semantically-similar or as semantically-dissimilar. The learned metric should place similar data points close to each other and far from the dissimilar ones. The training examples consist of two samples, $x_1$ and $x_2$ belonging to classes $y_1$ and $y_2$. The embedding representations produced by each network copy are $r_1=\text{Net}(x_1)$ and $r_2=\text{Net}(x_2)$. The learning goal can be expressed mathematically as:

\begin{equation*}
\label{eq:optimization_problem}
% d(x_1,x_2)= 
\begin{cases}
    \min d(r_1,r_2),& \text{if } y_1=y_2\\
    \max d(r_1,r_2),& \text{otherwise}
\end{cases}
\end{equation*}
where $d$ the euclidean distance.

This optimization problem can be solved using the \textit{contrastive loss} function~\cite{hadsell2006dimensionality,melekhov2016siamese}:
$$L(r_1,r_2,y)=y \cdot d(r1,r2)+(1-y)\max[0,m-d(r_1,r_2)]$$
where $y$ is a binary flag equal to 0 if $y_1=y_2$ and to 1 if $y_1\neq y_2$ and $m$ is a margin parameter. In particular, when $y_1\neq y_2$, $L=0$ when $d(r1,r2)\geq m$, otherwise the parameters of the network are updated to produce more distant representation for those two elements. The idea behind the use of the margin is that when the distance between pairs of different classes are large enough and at most $m$, there is no reason to update the network weights to place the representations even further away from each other and instead focus the training on harder examples.

==> tables/comparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht]
\centering
\caption{Evaluation metrics results}
\label{tab:taxonomy_comparison}
\begin{tabular}{|c|c|c|c|c|c|c|}
\cline{1-7}
               Dataset                       &        Taxonomy               & Accuracy & NLL        & BS     & ECE    & MCE    \\ \hline\hline
\multicolumn{1}{|c|}{\multirow{8}{*}{GTSRB}} & v1                            & 0.994    & 111.835    & 0.013  & 0.005  & 0.005  \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                       & v2                            & 0.992    & 58.104     & 0.055  & 0.011  & 0.583  \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                       & v3                            & 0.993    & 75.394     & 0.038  & 0.008  & 0.75   \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                       & v4                            & 0.991    & 70.279     & 0.053  & 0.009  & 0.75   \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                       & knn v1                        & 0.998    & 41.575     & 0.005  & 0.004  & 0.004  \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                       & knn v2                        & 0.998    & 41.126     & 0.005  & 0.004  & 0.004  \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                       & nc v1                         & 0.998    & 41.575     & 0.005  & 0.004  & 0.004  \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                       & nc v2                         & 0.996    & 38.444     & 0.046  & 0.007  & 0.5    \\ \hline\hline
\multicolumn{1}{|c|}{\multirow{8}{*}{BDD}}   & v1                            & 0.9199   & 12762.5697 & 0.1149 & 0.0014 & 0.0067 \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                       & v2                            & 0.9366   & 10749.6648 & 0.094  & 0.0013 & 0.0332 \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                       & v3                            & 0.9314   & 11277.0212 & 0.0994 & 0.0017 & 0.0481 \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                       & v4                            & 0.9349   & 10913.4966 & 0.0956 & 0.0015 & 0.0299 \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                       & knn v1                        & 0.9373   & 16349.4001 & 0.118  & 0.0005 & 0.0077 \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                       & knn v2                        & 0.9392   & 14488.1722 & 0.1051 & 0.0014 & 0.0166 \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                       & nc v1                         & 0.9235   & 11514.5642 & 0.1031 & 0.0014 & 0.006  \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                       & nc v2                         & 0.9256   & 11122.5832 & 0.1009 & 0.0015 & 0.0057 \\ \hline
\end{tabular}
\end{table*}
